When Context Leads but Parametric Memory Follows in Large Language Models

Large language models (LLMs) have demonstrated remarkable progress in leveraging diverse knowledge sources. This study investigates how nine widely used LLMs allocate knowledge between local context and global parameters when answering open-ended questions in knowledge-consistent scenarios. We introduce a novel dataset, WikiAtomic, and systematically vary context sizes to analyze how LLMs prioritize and utilize the provided information and their parametric knowledge in knowledge-consistent scenarios. Additionally, we also study their tendency to hallucinate under varying context sizes. Our findings reveal consistent patterns across models, including a consistent reliance on both contextual (around 70%) and parametric (around 30%) knowledge, and a decrease in hallucinations with increasing context. These insights highlight the importance of more effective context organization and developing models that use input more deterministically for robust performance.

==> latex/sections/discussion_newknowledgeplots.tex <==
\begin{itemize}
    \item \emph{Models process context very similarly} \quad This consistency was evident in how models balanced contextual and parametric knowledge, adjusted response lengths to match context lengths, included global facts, prioritized earlier context, and showed similar hallucination tendencies. This suggests a standardized approach to context processing.

    \item \emph{Balancing contextual and parametric knowledge} \quad Regardless of context size, models do not use all provided information, potentially leaving out critical details, and always included some parametric knowledge. As such there is a need to develop models that utilize input contexts more deterministically.

\item \emph{Order matters} \quad Models prioritize later information with smaller contexts and earlier information with larger contexts. Responses often follow the order of presented information, highlighting the importance of organizing context effectively.

\item \emph{Similar contextual knowledge but supplemental parametric knowledge} \quad Models tend to include similar contextual knowledge in their responses; parametric knowledge is initially diverse when context is minimal but becomes more aligned with the provided context as it increases, though it remains distinct from local knowledge. 

\item \emph{Increased context decreases hallucination.} \quad While the amount of parametric knowledge remains fairly consistent across context sizes, there is a noticeable improvement in the hallucination rate with increased context, implying that providing more context helps models generate more accurate responses, reducing reliance on potentially incorrect parametric knowledge.


\end{itemize}







\section{Prompt Analysis}\label{sec:ablation}



As shown in Figure~\ref{fig:new_gpt4o_main} and  {\ref{app:new_knowledge}}, we observed common patterns. 




\section{New knowledge}
\label{app:new_knowledge}

Figure \ref{fig:new_claude_gpt4o}, \ref{fig:new_llama3_mistralai} show how each behave when asking question about a new information. 

% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=0.6\textwidth]{figures/new_knowledge/new_gpt4o.png}
%     \caption{New knowledge (GPT-4o)}
%     \label{fig:new_gpt4o}
% \end{figure*} 

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/new_knowledge/new_gpt4o.png}
    \caption{New knowledge (GPT-4o)}
    \label{fig:new_gpt4o}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/new_knowledge/new_opus.png}
    \caption{New knowledge (Opus)}
    \label{fig:new_opus}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/new_knowledge/new_sonnet.png}
    \caption{New knowledge (Sonnet)}
    \label{fig:new_sonnet}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/new_knowledge/new_haiku.png}
    \caption{New knowledge (Haiku)}
    \label{fig:new_haiku}
    \end{subfigure}
    \caption{New knowledge (All Claude models)}
    \label{fig:new_claude_gpt4o}
\end{figure*} 

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/new_knowledge/new_llama370b.png}
    \caption{New knowledge (Llama 3 70B)}
    \label{fig:new_llama370b}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/new_knowledge/new_llama38b.png}
    \caption{New knowledge (Llama 3 8B)}
    \label{fig:new_llama38b}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/new_knowledge/new_mixtral.png}
    \caption{New knowledge (Mixtral 8x22B)}
    \label{fig:new_mixtral}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/new_knowledge/new_mistral.png}
    \caption{New knowledge (Mistral 7B)}
    \label{fig:new_mistral}
    \end{subfigure}
    \begin{subfigure}[t]{0.6\textwidth}
    \includegraphics[width=\textwidth]{figures/new_knowledge/new_phi.png}
    \caption{New knowledge (Phi 3)}
    \label{fig:new_phi}
    \end{subfigure}
    \caption{New knowledge (Phi 3, Mistral AI and Llama 3 models)}
    \label{fig:new_llama3_mistralai}
\end{figure*} 




\begin{figure}[t!]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/new_knowledge/new_gpt4o.png}
    \caption{New knowledge (GPT-4o)}
    \label{fig:new_gpt4o_main}
\end{figure}




==> options-packages.tex <==
% % This must be in the first 5 lines to tell arXiv to use pdfLaTeX, which is strongly recommended.
% \pdfoutput=1
% % In particular, the hyperref package requires pdfLaTeX in order to break URLs across lines.

% \documentclass[11pt]{article}

% % Change "review" to "final" to generate the final (sometimes called camera-ready) version.
% % Change to "preprint" to generate a non-anonymous version with page numbers.
% \usepackage[preprint]{acl}

% % Standard package includes
% \usepackage{times}
% \usepackage{latexsym}

% % For proper rendering and hyphenation of words containing Latin characters (including in bib files)
% \usepackage[T1]{fontenc}
% % For Vietnamese characters
% % \usepackage[T5]{fontenc}
% % See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets

% % This assumes your files are encoded as UTF8
% \usepackage[utf8]{inputenc}

% % This is not strictly necessary, and may be commented out,
% % but it will improve the layout of the manuscript,
% % and will typically save some space.
% \usepackage{microtype}

% % This is also not strictly necessary, and may be commented out.
% % However, it will improve the aesthetics of text in
% % the typewriter font.
% \usepackage{inconsolata}

% %Including images in your LaTeX document requires adding
% %additional package(s)
% \usepackage{graphicx}

% % Don't indent paragraphs

% % Don't indent paragraphs
% % \usepackage[parfill]{parskip}
% % \usepackage{amsmath}
% % \usepackage{tcolorbox}
% % \usepackage{xcolor}

% %\usepackage[parfill]{parskip}
% \usepackage{amsmath}
% \usepackage{xcolor}
% \usepackage{booktabs}
% \usepackage{colortbl}
% \usepackage{tcolorbox}
% \usepackage{tabularx}

% % For Tables
% % \usepackage{arydshln} % for \hdashline
% % \usepackage{array}
% % \usepackage{multirow}


% % \usepackage{booktabs}

% \definecolor{linebg}{HTML}{7AA2E3}
% \definecolor{headerbg}{HTML}{C0DEFF} % Hex code FFF9D0
% \definecolor{headertext}{HTML}{222831}
% \definecolor{rowtext}{HTML}{90C8AC}




% \usepackage{subcaption}


% \newtcolorbox{mybox}{fontupper=\footnotesize}

% \newcommand{\yt}[1]{\textcolor{orange}{#1}}
% \newcommand{\ah}[1]{\textcolor{blue}{AH: #1}}
% \newcommand{\eh}[1]{\textcolor{purple}{EH: #1}}
% \newcommand{\mee}[1]{\textcolor{red}{#1}}

